ZNorm: Z-Score Gradient Normalization Accelerating Skip-Connected Network Training without Architectural Modification

The rapid advancements in deep learning necessitate better training methods for deep neural networks (DNNs). As models grow in complexity, vanishing and exploding gradients impede performance, particularly in skip-connected architectures like Deep Residual Networks. We propose Z-Score Normalization for Gradient Descent (ZNorm), an innovative technique that adjusts only the gradients without modifying the network architecture to accelerate training and improve model performance. ZNorm normalizes the overall gradients, providing consistent gradient scaling across layers, effectively reducing the risks of vanishing and exploding gradients and achieving superior performance. Extensive experiments on CIFAR-10 and medical datasets confirm that ZNorm consistently outperforms existing methods under the same experimental settings. In medical imaging applications, ZNorm significantly enhances tumor prediction and segmentation accuracy, underscoring its practical utility. These findings highlight ZNorm's potential as a robust and versatile tool for enhancing the training and effectiveness of deep neural networks, especially in skip-connected architectures, across various applications.

==> contents/0-backup.tex <==

\section{Introduction}
\label{sec:intro}

This document serves as an example submission to ECCV \ECCVyear{}.
It illustrates the format authors must follow when submitting a paper. 
At the same time, it gives details on various aspects of paper submission, including preservation of anonymity and how to deal with dual submissions.
We advise authors to read this document carefully.

The document is based on Springer LNCS instructions as well as on ECCV policies, as established over the years.

\section{Initial Submission}

\subsection{Language}
All manuscripts must be in English.


\subsection{Template}
Papers must be prepared with the official LNCS style from Springer.
This applies to both review and camera-ready versions.
Springer requires manuscripts to be prepared in \LaTeX{} (strongly encouraged) or Microsoft Word. 

Authors preparing their paper with \LaTeX{} must use the template provided by ECCV, which is based on the corresponding Springer class file \texttt{llncs.cls} but includes line numbers for review (\cref{sec:line-numbering}) and properly anonymizes the paper for review (as in this example document).
Authors who -- for whatever reason -- cannot use \LaTeX{} can alternatively use the official LNCS Word template from Springer.
However, it is the authors' responsibility to ensure that the resulting PDF file is consistent with this example paper and follows it as closely as possible (\ie, includes line numbers, is properly anonymized, \etc).

We would like to stress that the class/style files and the template must not be manipulated and that the guidelines regarding font sizes and format must be adhered to. 
For example, please refrain from using any \LaTeX{} or \TeX{} command that modifies the layout settings of the template (\eg, \verb+\textheight+, \verb+\vspace+, \verb+\baselinestretch+, \etc).
Such manual layout adjustments should be limited to very exceptional cases.
This is to ensure that the end product is as homogeneous as possible.

Papers that differ significantly from the required style may be rejected without review.


\subsubsection{Fonts.}
Springer's templates for \LaTeX{} are based on CMR, and the XML templates for Word are based on Times. 
We ask you to use the font according to the template used for your papers. 
Specifically, please refrain from using Times when preparing your paper with \LaTeX{}.
Using a different font can be interpreted as purposely circumventing the length limitations and may lead to rejection without review.


\subsection{Paper Length}
Papers submitted for review must be complete. 
The length should match that intended for final publication. 
Papers accepted for the conference will be allocated 14 pages (plus additional pages for references) in the proceedings. 
Note that the allocated 14 pages do not include the references. 
The reason for this policy is that we do not want authors to omit references for sake of space limitations.

Papers with more than 14 pages (excluding references) will be rejected without review.
This includes papers where the margins and formatting including the font are deemed to have been significantly altered from those laid down by this style guide.

The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts. 
The reviewing process cannot determine the suitability of the paper for presentation in 14 pages if it is reviewed in 16.


\subsection{Paper ID}
It is imperative that the paper ID is mentioned on each page of the manuscript of the review version.
Enter your paper ID in the appropriate place in the \LaTeX{} template (see \texttt{\%TODO REVIEW}).
The paper ID is a number automatically assigned to your submission when registering your paper submission on the submission site.


\subsection{Line Numbering}
\label{sec:line-numbering}
All lines should be numbered in the initial submission, as in this example document. 
This makes reviewing more efficient, because reviewers can refer to a line on a page. 
Line numbering is removed in the camera-ready version.


\section{Policies}
The policies governing the review process of ECCV \ECCVyear{} are detailed on the conference webpage (see \url{https://eccv2024.ecva.net/}), such as regarding confidentiality, dual submissions, double-blind reviewing, plagiarism, and more. 
By submitting a paper to ECCV, the authors acknowledge that they have read the submission policies and that the submission follows the rules set forth.

Accepted papers will be published in LNCS proceedings with Springer.
To that end, authors must follow the Springer Nature Code of Conduct for Authors (see \url{https://www.springernature.com/gp/authors/book-authors-code-of-conduct}).
We would like to draw particular attention to the policies regarding figures and illustrations, as well as ethical approval and informed consent, which are also reproduced on the ECCV website.


\section{Preserving Anonymity}
\label{sec:blind}
ECCV reviewing is double blind, in that authors do not know the names of the area chair/reviewers of their papers, and the area chairs/reviewers cannot, beyond reasonable doubt, infer the names of the authors from the submission and the additional material. 
You must not identify the authors nor provide links to websites that identify the authors, neither in the paper nor in the supplemental material.
If you need to cite a different paper of yours that is being submitted concurrently to ECCV, you should \emph{(1)} cite these papers anonymously, \emph{(2)} argue in the body of your paper why your ECCV paper is non-trivially different from these concurrent submissions, and \emph{(3)} include anonymized versions of those papers in the supplemental material.
Violation of any of these guidelines may lead to rejection without review. 

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
  \begin{center}
      An analysis of the frobnicatable foo filter.
  \end{center}

   In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}

An example of an acceptable paper:
\begin{quote}
  \begin{center}
     An analysis of the frobnicatable foo filter.
  \end{center}

   In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission [1] as supplemental material and cite it as
\begin{quote}
  [1] Authors. ``The frobnicatable foo filter'', ECCV \ECCVyear Submission ID 00324, Supplied as supplemental material {\tt 00324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not \emph{require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Anonymous24b}''.
Then submit the tech report as supplemental material.
Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem, which you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the ECCV audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.

For sake of anonymity, authors must omit acknowledgements in the review copy. 
They can be added later when you prepare the final copy.


\section{Formatting Guidelines}

\subsection{Headings}
Headings should be capitalized (\ie, nouns, verbs, and all other words except articles, prepositions, and conjunctions should be set with an initial capital) and should, with the exception of the title, be aligned to the left.
Only the first two levels of section headings should be numbered, as shown in \cref{tab:headings}.
The respective font sizes are also given in \cref{tab:headings}. 
Kindly refrain from using ``0'' when numbering your section headings.
Words joined by a hyphen are subject to a special rule. 
If the first word can stand alone, the second word should be capitalized.

\begin{table}[tb]
  \caption{Font sizes of headings. 
    Table captions should always be positioned \emph{above} the tables.
  }
  \label{tab:headings}
  \centering
  \begin{tabular}{@{}lll@{}}
    \toprule
    Heading level & Example & Font size and style\\
    \midrule
    Title (centered)  & {\Large\bf Lecture Notes \dots} & 14 point, bold\\
    1st-level heading & {\large\bf 1 Introduction} & 12 point, bold\\
    2nd-level heading & {\bf 2.1 Printing Area} & 10 point, bold\\
    3rd-level heading & {\bf Headings.} Text follows \dots & 10 point, bold\\
    4th-level heading & {\it Remark.} Text follows \dots & 10 point, italic\\
  \bottomrule
  \end{tabular}
\end{table}

Here are some examples of headings: 
``Criteria to Disprove Context-Freeness of Collage Languages'', ``On Correcting the Intrusion of Tracing Non-deterministic Programs by Software'', ``A User-Friendly and Extendable Data Distribution System'', ``Multi-flip Networks: Parallelizing GenSAT'', ``Self-determinations of Man''.


\subsection{Figures}
\label{sect:figures}
For \LaTeX{} users, we recommend integrating figures in your paper using the package \texttt{graphicx}.

It is essential that all illustrations are clear and legible. 
Vector graphics (rather than rasterized images) should be used for diagrams and schemas whenever possible. 
Please check that the lines in line drawings are not interrupted and have a constant width. 
Line drawings are to have a resolution of at least 800 dpi (preferably 1200 dpi).
Grids and details within figures must be clearly legible and may not be written one on top of the other. 
The lettering in figures should not use font sizes smaller than 6\:pt ($\sim$2\:mm character height). 

Figures should be numbered and should have a caption, which should always be positioned \emph{under} the figures, in contrast to the caption belonging to a table, which should always appear \emph{above} the table.
Figures and Tables should be cross-referred in the text.

If they are short, they are centered between the margins (\cf \cref{fig:short}). 
Longer captions, covering more than one line, are justified (\cref{fig:example} shows an example). 
Captions that do not constitute a full sentence, do not have a period.


\begin{figure}[tb]
  \centering
  \includegraphics[height=6.5cm]{eijkel2}
  \caption{One kernel at $x_s$ (\emph{dotted kernel}) or two kernels at $x_i$ and $x_j$ (\emph{left and right}) lead to the same summed estimate at $x_s$.
    This shows a figure consisting of different types of lines.
    Elements of the figure described in the caption should be set in italics, in parentheses, as shown in this sample caption. 
    The last sentence of a figure caption should generally end with a full stop, except when the caption is not a full sentence.
  }
  \label{fig:example}
\end{figure}

\begin{figure}[tb]
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Centered, short example caption}
  \label{fig:short}
\end{figure}

If possible (\eg, if you use \LaTeX) please define figures as floating objects. 
\LaTeX{} users, please avoid using the location parameter ``h'' for ``here''. 
If you have to insert a pagebreak before a figure, please ensure that the previous page is completely filled.


\subsection{Formulas}
Displayed equations or formulas are centered and set on a separate line (with an extra line or half line space above and below). 
Equations should be numbered for reference. 
The numbers should be consecutive within the contribution, with numbers enclosed in parentheses and set on the right margin.
For example,
\begin{align}
  \psi (u) & = \int_{0}^{T} \left[\frac{1}{2}
  \left(\Lambda_{0}^{-1} u,u\right) + N^{\ast} (-u)\right] \text{d}t \; \\
& = 0
\end{align}
and 
\begin{equation}
  E = m\cdot c^2.
  \label{eq:important}
\end{equation}
Please do not include section counters in the numbering.

Numbering equations makes reviewing more efficient, because reviewers can refer to a line on a page.  
It is important for readers to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{https://doi.org/10.1063/1.2811173}.

% No color equations in Springer publications.
Equations should never be in color and should be punctuated in the same way as ordinary text.
They should not be pasted in as figures.


\subsubsection{Lemmas, Propositions, and Theorems.}
The numbers accorded to lemmas, propositions, and theorems, \etc should appear in consecutive order, starting with Lemma 1. 
Please do not include section counters in the numbering like ``Theorem 1.1''.


\subsection{Footnotes.}
The superscript numeral used to refer to a footnote appears in the text either directly after the word to be discussed or -- in relation to a phrase or a sentence -- following the punctuation mark (comma, semicolon, or period).%
\footnote{The footnote numeral is set flush left and the text follows with the usual word spacing. 
  Second and subsequent lines are indented. 
}
For remarks pertaining to the title or the authors' names, in the header of a paper, symbols should be used instead of a number.
Please note that no footnotes may be included in the abstract.


\subsection{Cross References}
For the benefit of author(s) and readers, please use the
\begin{verbatim}
  \cref{...}
\end{verbatim}
command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:example} and \cref{tab:headings}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:example,fig:short-a}.
  You may also return to \cref{sec:intro} or look at \cref{eq:important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
\begin{verbatim}
  \Cref{...}
\end{verbatim}
command. Here is an example:
\begin{quotation}
  \Cref{fig:example} is also quite important.
\end{quotation}


\subsection{Program Code}
Program listings or program commands in the text are normally set in typewriter font (\eg, \texttt{printf("Hello world!\textbackslash{}n");}).


\subsection{Citations}
Arabic numbers are used for citation, which is sequential either by order of citation or by alphabetical order of the references, depending on which sequence is used in the list of references. 
The reference numbers are given in brackets and are not superscript.
Please observe the following guidelines:
\begin{itemize}
\item Single citation: \cite{Anonymous24}
\item Multiple citation: \cite{Alpher02,Alpher03,Alpher05,Anonymous24b,Anonymous24}. 
  The numbers should be listed in numerical order.
  If you use the template as advised, this will be taken care of automatically.
\item If an author's name is used in the text: Alpher \cite{Alpher02} was the first \ldots
\end{itemize}
Please write all references using the Latin alphabet. If the title of the book you are referring to is, \eg, in Russian or Chinese, then please write (in Russian) or (in Chinese) at the end of the transcript or translation of the title.
All references cited in the text should be in the list of references and vice versa.

References should be formatted with the official LNCS reference style.
The \LaTeX{} template already takes care of that through the use of the \texttt{splncs04.bst} Bib\TeX{} style file.
Springer strongly encourages you to include DOIs (Digital Object Identifiers) in your references (\cf \cite{ECCV2022}). 
The DOI is a unique code allotted by the publisher to each online paper or journal article. 
It provides a stable way of finding published papers and their metadata. 
The insertion of DOIs increases the overall length of the references section, but this should not concern you as the reference section is not counted toward the page limit.


\subsection{Miscellaneous}
Compare the following:
\begin{center}
  \begin{tabular}{ll}
    \verb'$conf_a$'          & $\qquad conf_a$ \\
    \verb'$\mathit{conf}_a$' & $\qquad \mathit{conf}_a$
  \end{tabular}
\end{center}
See The \TeX book, p.\ 165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, \emph{e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', 
shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et\hskip 0.1em}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.


\section{Camera-Ready Manuscript Preparation}
\label{sec:manuscript}
This information will follow after paper decisions have been announced.


\section{Conclusion}
The paper ends with a conclusion. 

\clearpage\mbox{}Page \thepage\ of the manuscript.
\clearpage\mbox{}Page \thepage\ of the manuscript.
\clearpage\mbox{}Page \thepage\ of the manuscript.
\clearpage\mbox{}Page \thepage\ of the manuscript.
\clearpage\mbox{}Page \thepage\ of the manuscript. This is the last page.
\par\vfill\par
Now we have reached the maximum length of an ECCV \ECCVyear{} submission (excluding references).
References should start immediately after the main text, but can continue past p.\ 14 if needed.

==> contents/2-related_backup.tex <==
% Optimization techniques are central to training deep neural networks efficiently. Stochastic gradient descent (SGD) and its variants, such as SGD with momentum \citep{qian1999momentum} and adaptive methods like Adam \citep{kingma2014adam}, have been crucial in optimizing complex architectures. These methods minimize the loss function via parameter updates, with adaptive methods like Adagrad \citep{duchi2011adaptive} and RMSProp \citep{tieleman2012lecture} dynamically adjusting learning rates based on gradient magnitude and history.

% Normalization techniques address training instability and are essential for smoothing optimization landscapes. Batch normalization (BN) \citep{ioffe2015batch} normalizes activations based on mini-batch statistics. Layer normalization (LN) \citep{ba2016layer} and group normalization (GN) \citep{wu2018group} handle different axes and combinations, while weight normalization (WN) \citep{salimans2016weightnorm} and weight standardization (WS) \citep{qiao2019weight} ensure consistent weight scaling. Gradient clipping \citep{clip} caps gradient magnitudes to prevent exploding gradients in recurrent networks. Weight decay applies L2 regularization \citep{krogh1991simple} to constrain weight growth. Gradient centralization~\citep{center} normalizes gradients to have zero mean, improving convergence and generalization.

% Our proposed Z-Score Normalization (ZNorm) builds on these techniques. By applying Z-score normalization directly to overall gradients, we standardize gradient scaling across layers, reducing vanishing and exploding gradients~\cite{pascanu2013difficulty} while ensuring consistent learning progress. This leads to improved generalization and robustness of the models. 

Optimization techniques are central to training deep neural networks effectively. Stochastic gradient descent (SGD) and its variants, such as SGD with momentum \citep{qian1999momentum} and adaptive methods like Adam \citep{kingma2014adam}, have been crucial in optimizing complex architectures. These methods aim to minimize the loss function via parameter updates. Adaptive optimizers like Adagrad \citep{duchi2011adaptive} and RMSProp \citep{tieleman2012lecture} further adjust learning rates dynamically based on gradient magnitude and history, stabilizing the training process for deep models. AdamW \citep{adamw} improves upon traditional weight decay by decoupling L2 regularization from the gradient update in adaptive optimization methods like Adam. In traditional Adam, weight decay is applied implicitly through the L2 regularization term, which affects both the gradient and the parameter updates. AdamW, however, applies weight decay directly to the weights during the parameter update step, ensuring that the regularization only affects the weight magnitudes and not the gradient direction. The gradient update for weight decay in AdamW is modified as $\nabla_\theta L_{\text{decay}}(\theta_t) = \nabla_\theta L(\theta_t) + \lambda \theta_t$ where $\lambda$ is the weight decay coefficient. This decoupled approach in AdamW prevents the regularization term from interfering with the adaptive learning rate updates, leading to more stable training and better generalization, especially in large-scale models. 

% \section{Related Works}
Training deep neural networks (DNNs) effectively requires overcoming challenges such as vanishing and exploding gradients, which hinder the performance of complex models~\citep{Pascanu2013}. Traditional approaches to address these issues include normalization techniques applied to activations and weights, such as Batch Normalization (BN)~\citep{ioffe2015batch}, Layer Normalization (LN)~\citep{ba2016layer}, and Weight Standardization (WS)~\citep{qiao2019weight}. While effective, these techniques require modifications to the network architecture, which can add complexity and limit flexibility. Additionally, large-batch optimization techniques, such as LARS~\citep{lamb} and LAMB~\citep{lars}, provide layer-wise adaptive learning rates, enabling stable training with large batches. While these methods effectively scale learning rates based on weight norms, they are primarily designed for large-batch settings and may not generalize to smaller batch sizes or different architectures. In contrast, ZNorm enhances training stability through direct gradient normalization, eliminating the need for complex adjustments or specific batch configurations. Unlike batch-dependent methods, ZNorm performs normalization on the gradient tensors themselves, ensuring consistent behavior regardless of the chosen batch size. 

Gradient adjustment methods directly manipulate the gradient updates to improve training stability and prevent issues like exploding or vanishing gradients. Gradient Clipping~\citep{pascanu2013difficulty} is one such method that caps gradient magnitudes to a threshold $\tau$, effectively preventing the exploding gradient problem. If the gradient exceeds $\tau$, it is rescaled like $\nabla_\theta L(\theta_t) \leftarrow \nabla_\theta L(\theta_t) \cdot \min\left(1, \frac{\tau}{||\nabla_\theta L(\theta_t)||}\right)$. While Gradient Clipping is effective for stabilizing training, it lacks comprehensive control over gradient distribution across layers, potentially leading to inconsistencies in gradient scaling. Gradient Centralization (GC)~\citep{center} is another method that normalizes gradients by zero-centering them, effectively enhancing training consistency and performance. GC achieves this by adjusting the gradient mean to zero $\nabla_\theta L(\theta_t) \leftarrow \nabla_\theta L(\theta_t) - \frac{1}{n} \sum_{i=1}^{n} \nabla_{\theta_i} L(\theta_t)$ where $n$ is the number of gradient elements. Although GC improves generalization and speeds up convergence, it only adjusts the mean, leaving the variance uncontrolled, which may not fully stabilize training in deep networks. SING~\citep{courtois2023sing} is another recent approach, offering plug-and-play gradient standardization to improve stability with optimizers such as AdamW. SING normalizes gradients layer-wise, enhancing generalization and allowing escape from narrow local minima. However, SING’s layer-wise adjustments are dependent on specific optimizers and introduce additional hyperparameters, whereas ZNorm operates independently of optimizer choice and requires no extra tuning, making it simpler to implement.

Building on these approaches, our work introduces Z-score Gradient Normalization (ZNorm), a technique that standardizes both the mean and variance of gradients across layers, ensuring consistent scaling. By normalizing the gradients using Z-scores, ZNorm directly addresses both vanishing and exploding gradients, particularly enhancing stability in skip-connected architectures like ResNet and U-Net. Unlike GC, which only zero-centers the gradient, ZNorm performs full normalization $\nabla_\theta L(\theta_t) \leftarrow \frac{\nabla_\theta L(\theta_t) - \mu_{\nabla}}{\sigma_{\nabla}}$ where $\mu_{\nabla}$ and $\sigma_{\nabla}$ are the mean and standard deviation of the gradient elements, respectively. This additional variance control provides more stable training across diverse skip-connected architectures and applications.


\begin{figure*}
  \centering
  \includegraphics[width=0.95\textwidth]{contents/main-str.png}
  \caption{Visualization of the ZNorm($\Phi$) process applied to gradient matrices and tensors in both fully-connected and convolutional layers. The process includes calculating the gradient mean vector and standard deviation vector, followed by normalizing the gradients via ZNorm.  The training process showing how normalized gradients $\Phi(\nabla L(\theta))$ are integrated into the forward-backward optimization loop, with gradient adjustment occurring between gradient computation and the optimizer update step.}
  \label{fig:main}
\end{figure*}

In summary, ZNorm positions itself as a straightforward and adaptable gradient normalization technique that avoids architectural modifications. By focusing solely on gradient adjustments, ZNorm can be easily integrated into various training processes with minimal changes. This layer-wise gradient scaling achieves stable and efficient training, particularly enhancing performance in skip-connected networks such as ResNet, DenseNet, and U-Net. As a result, ZNorm proves to be a valuable tool for improving training speed and effectiveness across diverse applications.

Furthermore, by only adjusting the gradients, ZNorm simplifies the training pipeline, making it suitable for rapid implementation without the need for extensive reconfiguration or additional hyperparameters. This adaptability allows ZNorm to be applied flexibly across different network architectures and tasks, ensuring that stable training benefits are accessible without requiring fundamental changes to the underlying model design.



==> contents/3-method.tex <==
Normalization techniques are crucial for stabilizing and enhancing the training of deep neural networks~\cite{}. This section introduces Z-Score Normalization (ZNorm), a technique designed to standardize gradient tensors across all network layers. ZNorm addresses the common challenges of gradient scaling, such as exploding~\cite{} or vanishing gradients~\cite{}, by ensuring consistent gradient magnitudes during training. This leads to improved convergence and robustness of the models. The following subsections will outline the detailed notations and mathematical framework that facilitate the application of ZNorm in neural network training.

\subsection{Notations}
To formalize the approach of Z-Score Normalization (ZNorm) within deep neural network training, we introduce comprehensive notations that will be used throughout this paper. Consider a deep neural network consisting of \(L\) layers, where each layer \(l\) has associated weights \(\mathbf{\theta}^{(l)}\). For fully connected layers, \(\mathbf{\theta}^{(l)} \in \mathbb{R}^{D_l \times M_l}\), with \(D_l\) representing the number of neurons and \(M_l\) the dimension of input to the layer. For convolutional layers, \(\mathbf{\theta}^{(l)}\) can be represented as a 4-dimensional tensor \(\mathbf{\theta}^{(l)} \in \mathbb{R}^{C_{out}^{(l)} \times C_{in}^{(l)} \times k_1^{(l)} \times k_2^{(l)}}\), where \(C_{in}^{(l)}\) and \(C_{out}^{(l)}\) are the number of input and output channels, respectively, and \(k_1^{(l)}\), \(k_2^{(l)}\) represent the kernel sizes. Let \(\nabla \mathbf{\theta}^{(l)}\) denote the gradient of the loss function with respect to the weights \(\mathbf{\theta}^{(l)}\) of layer \(l\). For fully connected layers, \(\nabla \mathbf{\theta}^{(l)} \in \mathbb{R}^{D_l \times M_l}\), and for convolutional layers, \(\nabla \mathbf{\theta}^{(l)} \in \mathbb{R}^{C_{out}^{(l)} \times C_{in}^{(l)} \times k_1^{(l)} \times k_2^{(l)}}\).

\subsection{Z-Score Normalization of Gradients}
The process of Z-Score Normalization is applied directly to the gradient tensors. Each gradient tensor \(\nabla \mathbf{\theta}^{(l)}\) is standardized as follows:

\begin{equation}
\Phi_{ZNorm}(\nabla w_i \mathcal{L}) =  \frac{\nabla w_i \mathcal{L} - \mu_{\nabla w_i \mathcal{L}}}{\sigma_{\nabla w_i \mathcal{L}} + \epsilon}
\end{equation}

Here, the mean gradient for layer $l$, denoted $\mu_{\nabla \mathbf{\theta}^{(l)}}$, is computed as:

\begin{equation}
    \mu_{\nabla \mathbf{\theta}^{(l)}} = \frac{1}{n^{(l)}} \sum_{i=1}^{n^{(l)}} \nabla \theta_i^{(l)}
\end{equation}


where $n^{(l)}$ is the total number of elements in $\nabla \mathbf{\theta}^{(l)}$ and $\nabla \theta_i^{(l)}$ denotes the $i$-th element of the flattened gradient tensor. The variance for layer $l$, denoted $\sigma^2_{\nabla \mathbf{\theta}^{(l)}}$, is calculated as $\sigma^2_{\nabla \mathbf{\theta}^{(l)}} = \frac{1}{n^{(l)}} \sum_{i=1}^{n^{(l)}} (\nabla \theta_i^{(l)} - \mu_{\nabla \mathbf{\theta}^{(l)}})^2$. To prevent division by zero \(\epsilon\) is a small constant, which is typically 1e-8.

\subsection{Stability of ZNorm Training}

% \section*{Analyzing the Scaling Effect}

Let's analyze the effect of \(\sigma_{\nabla w_i \mathcal{L}}\) on the gradient updates. We consider two cases: when \(\sigma_{\nabla w_i \mathcal{L}} < 1\) and when \(\sigma_{\nabla w_i \mathcal{L}} > 1\).

\subsection*{Case 1: \(\sigma_{\nabla w_i \mathcal{L}} < 1\)}

When the standard deviation \(\sigma_{\nabla w_i \mathcal{L}}\) is less than 1, the denominator \(\sigma_{\nabla w_i \mathcal{L}} + \epsilon\) will be small. This results in the normalized gradient being scaled up:
\[
\frac{1}{\sigma_{\nabla w_i \mathcal{L}} + \epsilon} > 1 \quad \text{if} \quad \sigma_{\nabla w_i \mathcal{L}} < 1
\]

Thus, the magnitude of the update becomes larger than the original gradient:
\[
\eta \frac{\nabla w_i \mathcal{L} - \mu_{\nabla w_i \mathcal{L}}}{\sigma_{\nabla w_i \mathcal{L}} + \epsilon} \quad \text{is larger than} \quad \eta \nabla w_i \mathcal{L}
\]

This can lead to excessively large updates, making the training process unstable or causing divergence.

\subsection*{Case 2: \(\sigma_{\nabla w_i \mathcal{L}} > 1\)}

When the standard deviation \(\sigma_{\nabla w_i \mathcal{L}}\) is greater than 1, the denominator \(\sigma_{\nabla w_i \mathcal{L}} + \epsilon\) will be large. This results in the normalized gradient being scaled down:
\[
\frac{1}{\sigma_{\nabla w_i \mathcal{L}} + \epsilon} < 1 \quad \text{if} \quad \sigma_{\nabla w_i \mathcal{L}} > 1
\]

Thus, the magnitude of the update becomes smaller than the original gradient:
\[
\eta \frac{\nabla w_i \mathcal{L} - \mu_{\nabla w_i \mathcal{L}}}{\sigma_{\nabla w_i \mathcal{L}} + \epsilon} \quad \text{is smaller than} \quad \eta \nabla w_i \mathcal{L}
\]

This can lead to very small updates, slowing down the convergence of the training process.


% \subsection{Integration into the Optimization Process}
% The normalized gradients are then used to update the weights during the training process:
% \begin{equation}
% \mathbf{\theta}^{(l)}_{t+1} = \mathbf{\theta}^{(l)}_{t} - \eta \cdot \nabla \mathbf{\theta}^{(l)}_{\text{z}}
% \end{equation}
% where \(\eta\) is the learning rate. This ensures that the updates are consistently scaled across all layers, promoting a more stable and efficient training process.

\subsubsection{\ho{Role of skip connection}}
ZNorm is stable in architectures with skip connections. ZNorm can prevent gradient vanishing. However, this characteristic can actually hinder learning. Towards the end of training, gradients theoretically converge to zero. However, due to the normalization of ZNorm, this convergence is obstructed. Therefore, there is a possibility of divergence at the end of training.

Skip connections can resolve this challenge. According to the chain rule of backpropagation, the gradient can be presented by the following equation:
\[
\nabla w_i \mathcal{L} = g_{0 \sim l-1} \cdot g_{l}
\]
where \( g_{l} \) is the derivative of layer \( l \), and \( g_{0 \sim l-1} \) is the accumulated derivative up to layer \( l \).

When skip connections are applied, the gradient can be presented as:
\[
\nabla w_i \mathcal{L} = g_{0 \sim l-1} \cdot (g_{l} + 1)
\]
This prevents the gradient from becoming extremely small, thereby enhancing the training stability of ZNorm.




==> contents/3-theory.tex <==
Z-score normalization normalizes gradients by subtracting their mean and dividing by the standard deviation, potentially altering the direction of individual components. This raises concerns about whether the overall descent direction is maintained. This analysis explains why, despite these changes, the optimization process remains effective. Specifically, it shows that the inner product of the normalized gradient with the original gradient remains positive, preserving the overall descent direction necessary for reducing the objective function. \\


\noindent \textbf{Lemma 4.1.} Let \( \nabla \mathcal{L}(\mathbf{\theta^{(l)}}) \in \mathbb{R}^d \) be the original gradient vector with mean \( \mu_{\nabla \mathcal{L}(\mathbf{\theta^{(l)}})} = \frac{1}{d} \sum_{i=1}^d \nabla \mathcal{L}(\mathbf{\theta_{i}^{(l)}}) \), variance \( \sigma_{\nabla \mathcal{L}(\mathbf{\theta^{(l)}})}^2 = {\frac{1}{d} \sum_{i=1}^d (\nabla \mathcal{L}(\mathbf{\theta_{(i)}^{(l)}}) - \mu_{\nabla \mathcal{L}(\mathbf{\theta^{(l)}})})^2} \). The Z-score normalized gradient \( \Phi_{Z}(\nabla \mathcal{L}(\mathbf{\theta_{(i)}^{(l)}})) \) is defined as
\[
\Phi_{Z}(\nabla \mathcal{L}(\mathbf{\theta_{(i)}^{(l)}})) = \frac{\nabla \mathcal{L}(\mathbf{\theta_{(i)}^{(l)}}) - \mu_{\nabla \mathcal{L}(\mathbf{\theta^{(l)}})}}{\sigma_{\nabla \mathcal{L}(\mathbf{\theta^{(l)}})}}
\]
 $\text{for } i = 1, 2, \dots, d.$ \\
Then, the inner product of the normalized gradient \( \Phi_{Z} \) with the original gradient \( \nabla \mathcal{L}(\mathbf{\theta^{(l)}}) \) is given by
\[
(\Phi_{Z})^T \nabla \mathcal{L}(\mathbf{\theta^{(l)}}) = \frac{\|\nabla \mathcal{L}(\mathbf{\theta^{(l)}})\|_2^2 - d \mu_\nabla \mathcal{L}(\mathbf{\theta^{(l)}})^2}{\sigma_\nabla \mathcal{L}(\mathbf{\theta^{(l)}})},
\]
where \( \|\nabla \mathcal{L}(\mathbf{\theta^{(l)}})\|_2 \) is the Euclidean norm of the vector \( \nabla \mathcal{L}(\mathbf{\theta^{(l)}}) \). This result indicates that while the Z-score standardization can alter the direction of individual components of the gradient, the overall descent direction is preserved. \\

\noindent \textbf{\textit{Proof.}} We begin by recalling the definition of the Z-score standardized gradient:
\[
\Phi_{Z}(\nabla \mathcal{L}(\mathbf{\theta_{(i)}^{(l)}})) = \frac{\nabla \mathcal{L}(\mathbf{\theta_{(i)}^{(l)}}) - \mu_{\nabla \mathcal{L}(\mathbf{\theta^{(l)}})}}{\sigma_{\nabla \mathcal{L}(\mathbf{\theta^{(l)}})}}.
\]
where  $\mu_{\nabla \mathcal{L}(\mathbf{\theta^{(l)}})} = \frac{1}{d} \sum_{i=1}^d \nabla \mathcal{L}(\mathbf{\theta_{(i)}^{(l)}}) \quad \text{and} \quad \sigma_{\nabla \mathcal{L}(\mathbf{\theta^{(l)}})}^2 = \frac{1}{d} \sum_{i=1}^d (\nabla \mathcal{L}(\mathbf{\theta_{(i)}^{(l)}}) - \mu_{\nabla \mathcal{L}(\mathbf{\theta^{(l)}})})^2$
Here, \( \mu_{\nabla \mathcal{L}(\mathbf{\theta^{(l)}})} \) represents the mean of the gradient components, and \( \sigma_{\nabla \mathcal{L}(\mathbf{\theta^{(l)}})} \) represents the standard deviation, which measures the spread of the gradient components around the mean.




Next, the z-score normalized gradient vector \( \Phi_{Z} \) can be expressed in vector form as:
\[
\Phi_{Z} = \frac{1}{\sigma_{\nabla \mathcal{L}(\mathbf{\theta^{(l)}})}} (\nabla \mathcal{L}(\mathbf{\theta^{(l)}}) - \mu_{\nabla \mathcal{L}(\mathbf{\theta^{(l)}})} \mathbf{1}),
\]
where \( \mathbf{1} \) is the \( d \)-dimensional vector of ones.

Here, the inner product \( (\Phi_{Z})^T\nabla \mathcal{L}(\mathbf{\theta^{(l)}}) \), which is given by:
\[
(\Phi_{Z})^T \nabla \mathcal{L}(\mathbf{\theta^{(l)}}) = \left( \frac{(\nabla \mathcal{L}(\mathbf{\theta^{(l)}}) - \mu_{\nabla \mathcal{L}(\mathbf{\theta^{(l)}})} \mathbf{1}) }{\sigma_{\nabla \mathcal{L}(\mathbf{\theta^{(l)}})}}\right)^T\nabla \mathcal{L}(\mathbf{\theta^{(l)}}).
\]
Expanding this expression, we get:
\begin{align}
    (\Phi_{Z})^T\nabla \mathcal{L}(\mathbf{\theta^{(l)}}) &= \frac{( (\nabla \mathcal{L}(\mathbf{\theta^{(l)}}))^T \nabla \mathcal{L}(\mathbf{\theta^{(l)}})}{\sigma_{\nabla \mathcal{L}(\mathbf{\theta^{(l)}})}} \\
    &- \frac{- \mu_{\nabla \mathcal{L}(\mathbf{\theta^{(l)}})} \mathbf{1}^T {\nabla \mathcal{L}(\mathbf{\theta^{(l)}})} )}{\sigma_{\nabla \mathcal{L}(\mathbf{\theta^{(l)}})}}
\end{align}
Now, we calculate \( \mathbf{1}^T \nabla \mathcal{L}(\mathbf{\theta^{(l)}}) \), which represents the sum of all components of the gradient vector \( \nabla \mathcal{L}(\mathbf{\theta^{(l)}}) \):
\[
\mathbf{1}^T \nabla \mathcal{L}(\mathbf{\theta^{(l)}}) = \sum_{i=1}^d \nabla \mathcal{L}(\mathbf{\theta_{(i)}^{(l)}}) = d \mu_{\nabla \mathcal{L}(\mathbf{\theta^{(l)}})}.
\]
Substituting this into the expression for \( (\Phi_{Z})^T \nabla \mathcal{L}(\mathbf{\theta^{(l)}}) \), we obtain:
\[
(\Phi_{Z})^T \nabla \mathcal{L}(\mathbf{\theta^{(l)}}) = \frac{(\nabla \mathcal{L}(\mathbf{\theta^{(l)}}))^T \nabla \mathcal{L}(\mathbf{\theta^{(l)}}) - d \mu_{\nabla \mathcal{L}(\mathbf{\theta^{(l)}})}^2}{\sigma_{\nabla \mathcal{L}(\mathbf{\theta^{(l)}})}}  .
\]
Next, let's express \( (\Phi_{Z})^T \nabla \mathcal{L}(\mathbf{\theta^{(l)}}) \) in terms of the Euclidean norm of \( \nabla \mathcal{L}(\mathbf{\theta^{(l)}}) \):
\[
(\Phi_{Z})^T \nabla \mathcal{L}(\mathbf{\theta^{(l)}}) = \sum_{i=1}^d (\nabla \mathcal{L}(\mathbf{\theta_{(i)}^{(l)}}))^2 = \|\nabla \mathcal{L}(\mathbf{\theta^{(l)}})\|_2^2.
\]



Thus, the inner product becomes:
\[
(\Phi_{Z})^T \nabla \mathcal{L}(\mathbf{\theta^{(l)}}) = \frac{\|\nabla \mathcal{L}(\mathbf{\theta^{(l)}})\|_2^2 - d \mu_{\nabla \mathcal{L}(\mathbf{\theta^{(l)}})}^2}{\sigma_{\nabla \mathcal{L}(\mathbf{\theta^{(l)}})}}.
\]
This equation shows that the inner product of the Z-score normalized gradient \( \Phi_{Z} \) with the original gradient \( \nabla \mathcal{L}(\mathbf{\theta^{(l)}}) \) is determined by the difference between the squared Euclidean norm of \( \nabla \mathcal{L}(\mathbf{\theta^{(l)}}) \) and the scaled mean squared value of \( \nabla \mathcal{L}(\mathbf{\theta^{(l)}}) \), divided by the standard deviation \( \sigma_{\nabla \mathcal{L}(\mathbf{\theta^{(l)}})} \).

This result is significant because it indicates that while the Z-score standardization can change the direction of individual components of the gradient, the overall directionality, as measured by the inner product \( (\Phi_{Z})^T \nabla \mathcal{L}(\mathbf{\theta^{(l)}}) \), remains aligned with the original gradient direction. Specifically, if \( \nabla \mathcal{L}(\mathbf{\theta^{(l)}}) \) is a descent direction, then \( (\Phi_{Z})^T \) will also be a descent direction, as the inner product \( (\Phi_{Z})^T \nabla \mathcal{L}(\mathbf{\theta^{(l)}})\) remains positive, which proves the lemma. \\


\noindent \textbf{Theorem 4.2.} Given the same conditions as in the Lemma, the Z-score normalized gradient \( \hat{g} \) preserves the descent direction of the original gradient \( \nabla \mathcal{L}(\mathbf{\theta^{(l)}}) \). Specifically, if \( \nabla \mathcal{L}(\mathbf{\theta^{(l)}}) \) is a descent direction, then \( (\Phi_{Z}) \) is also a descent direction, i.e.,
\[
(\Phi_{Z})^T \nabla \mathcal{L}(\mathbf{\theta^{(l)}}) > 0.
\]
This implies that even though Z-score standardization may change the directions of individual gradient components, the overall gradient vector still points in a direction that will reduce the objective function. \\





\noindent \textbf{\textit{Proof.}} From the result of the Lemma, we have:
\[
(\Phi_{Z})^T \nabla \mathcal{L}(\mathbf{\theta^{(l)}}) = \frac{\|\nabla \mathcal{L}(\mathbf{\theta^{(l)}})\|_2^2 - d \mu_{\nabla \mathcal{L}(\mathbf{\theta^{(l)}})}^2}{\sigma_{\nabla \mathcal{L}(\mathbf{\theta^{(l)}})}}.
\]
Here, \( \|\nabla \mathcal{L}(\mathbf{\theta^{(l)}})\|_2^2 = \sum_{i=1}^d \nabla \mathcal{L}(\mathbf{\theta_{(i)}^{(l)}})^2 \) is the squared Euclidean norm of the gradient vector \( \nabla \mathcal{L}(\mathbf{\theta^{(l)}}) \), and \( \mu_{\nabla \mathcal{L}(\mathbf{\theta^{(l)}})} \) is the mean of the gradient components.

Since \( \sigma_{\nabla \mathcal{L}(\mathbf{\theta^{(l)}})} \) is the standard deviation of the elements of \( \nabla \mathcal{L}(\mathbf{\theta^{(l)}}) \), we have \( \sigma_{\nabla \mathcal{L}(\mathbf{\theta^{(l)}})} > 0 \). The standard deviation \( \sigma_{\nabla \mathcal{L}(\mathbf{\theta^{(l)}})} \) is positive as long as the components of \( \nabla \mathcal{L}(\mathbf{\theta^{(l)}}) \) are not all identical (i.e., \( g_i \) are not constant for all \( i \)).

Next, consider the term \( d \mu_{\nabla \mathcal{L}(\mathbf{\theta^{(l)}})}^2 \). This term can be rewritten as:
\[
d \mu_{\nabla \mathcal{L}(\mathbf{\theta^{(l)}})}^2 = d \left( \frac{1}{d} \sum_{i=1}^d \nabla \mathcal{L}(\mathbf{\theta_{(i)}^{(l)}}) \right)^2 = \frac{1}{d} \left( \sum_{i=1}^d \nabla \mathcal{L}(\mathbf{\theta_{(i)}^{(l)}}) \right)^2.
\]
This expression represents the squared mean of the gradient components scaled by the dimension \( d \). Now, by the Cauchy-Schwarz inequality, we have:
\[
\sum_{i=1}^d \nabla \mathcal{L}(\mathbf{\theta_{(i)}^{(l)}})^2 \geq \frac{1}{d} \left( \sum_{i=1}^d \nabla \mathcal{L}(\mathbf{\theta_{(i)}^{(l)}}) \right)^2 = d \mu_{\nabla \mathcal{L}(\mathbf{\theta^{(l)}})}^2.
\]
This inequality ensures that the term \( \|\nabla \mathcal{L}(\mathbf{\theta^{(l)}})\|_2^2 - d \mu_{\nabla \mathcal{L}(\mathbf{\theta^{(l)}})}^2 \) is non-negative:
\[
\|\nabla \mathcal{L}(\mathbf{\theta^{(l)}})\|_2^2 - d \mu_{\nabla \mathcal{L}(\mathbf{\theta^{(l)}})}^2 \geq 0.
\]
Therefore, the inner product \( (\Phi_{Z})^T  \nabla \mathcal{L}(\mathbf{\theta^{(l)}}) \) can be expressed as:
\[
(\Phi_{Z})^T \nabla \mathcal{L}(\mathbf{\theta^{(l)}})= \frac{\|\nabla \mathcal{L}(\mathbf{\theta^{(l)}})\|_2^2 - d \mu_{\nabla \mathcal{L}(\mathbf{\theta^{(l)}})}^2}{\sigma_{\nabla \mathcal{L}(\mathbf{\theta^{(l)}})}} \geq 0.
\]






For \( \hat{g}^T g \) to be strictly positive, \( \nabla \mathcal{L}(\mathbf{\theta^{(l)}}) \) must not be a constant vector (i.e., not all \( \nabla \mathcal{L}(\mathbf{\theta_{(i)}^{(l)}}) \) are the same), ensuring that \( \sigma_{\nabla \mathcal{L}(\mathbf{\theta^{(l)}})} > 0 \) and \( \|\nabla \mathcal{L}(\mathbf{\theta^{(l)}})\|_2^2 > d \mu_{\nabla \mathcal{L}(\mathbf{\theta^{(l)}})}^2 \). This condition holds under typical scenarios in optimization where the gradient vector \( \nabla \mathcal{L}(\mathbf{\theta^{(l)}}) \) varies across its components. The above proof shows that \( (\Phi_{Z})^T \nabla \mathcal{L}(\mathbf{\theta^{(l)}}) \) is positive under general conditions, but it may not always be positive in specific cases. Particularly, if all components of the gradient are identical (i.e., \( \nabla \mathcal{L}(\mathbf{\theta_{(i)}^{(l)}}) = \text{constant} \)), the standard deviation \( \sigma_{\nabla \mathcal{L}(\mathbf{\theta^{(l)}})} = 0 \), making the inner product undefined or zero. Therefore, while Z-score standardization generally preserves the descent direction in typical scenarios, it may not always do so in extreme cases. Therefore, under these conditions, \( (\Phi_{Z})^T \nabla \mathcal{L}(\mathbf{\theta^{(l)}}) > 0 \), which implies that the Z-score normalized gradient \( (\Phi_{Z}) \) indeed preserves the descent directionality. Despite the potential changes in individual components caused by Z-score standardization, the overall direction of the gradient vector \( \nabla \mathcal{L}(\mathbf{\theta^{(l)}}) \) that leads to a decrease in the objective function is preserved, proving the theorem.


% \begin{figure*}
%   \centering
%   \includegraphics[width=1.0\textwidth]{contents/CIFAR10.png}
%   \caption{Test Accuracy on CIFAR-10~\cite{Krizhevsky2009LearningML} for Skip-Connected Networks (ResNet-152~\cite{He2016DeepRL} and DenseNet-169~\cite{Huang2017DenselyCC}) and Non-Skip-Connected Network (Xception~\cite{Chollet2017XceptionDL}) over 100 epochs using various normalization techniques based on Adam~\cite{kingma2014adam}: Gradient Centralization~\cite{center}, Gradient Clipping~\cite{clip}, Baseline, and ZNorm (Ours).}
%   \label{fig:testac}
% \end{figure*}


==> contents/4-3-PATCHWISE.tex <==
\subsubsection{Patch-Wise Tumor Prediction}

\begin{table}[htbp]
\centering
\tiny
\caption{Performance Comparison of Tumor Prediction}
\begin{adjustbox}{width=1\textwidth}
\begin{tabular}{|l|l|lcc|}
\hline
Datasets & Model & Methods & Train Loss & Test Accuracy \\
\# of classes & (\# of Params.) &&& \\
\hline
\hline

& \multirow{6}{*}{ResNet-56 (0.86M)~\cite{He2016DeepRL}}
& Baseline & 0.802 & 0.0033 \\
&& Gradient Centralization & 0.804 & 0.0128 \\
&& Gradient Clipping & 0.747 & 0.0178 \\
&& Weight Decay 1E-3~\cite{adamw} & - & - \\
&& Weight Decay 1E-4~\cite{adamw} & - & - \\
&& ZNorm (Ours) & \textbf{0.812} & 0.0178 \\
\cline{2-5} 
& \multirow{6}{*}{ResNet-110 (0.86M)~\cite{He2016DeepRL}}
& Baseline & 0.770 & 0.0165 \\
PatchCamelyon~\cite{pcam} & & Gradient Centralization & 0.813 & 0.0112 \\
(2) & & Gradient Clipping & 0.772 & 0.0152 \\
&& Weight Decay 1E-3~\cite{adamw} & - & - \\
&& Weight Decay 1E-4~\cite{adamw} & - & - \\
& & ZNorm (Ours) & \textbf{0.820} & 0.0160 \\
\cline{2-5} 
& \multirow{6}{*}{ResNet-152 (0.86M)~\cite{He2016DeepRL}}
& Baseline & 0.795 & 0.0172 \\
&& Gradient Centralization & 0.797 & 0.0246 \\
&& Gradient Clipping & 0.786 & 0.0311 \\
&& Weight Decay 1E-3~\cite{adamw} & - & - \\
&& Weight Decay 1E-4~\cite{adamw} & - & - \\
&& ZNorm (Ours) & \textbf{0.823} & 0.0217 \\

\hline
\end{tabular}
\label{tab:cnn}
\end{adjustbox}
\end{table}


==> contents/6-1-theorem1.tex <==
\noindent \textbf{Lemma 6.1.} Let \( g \in \mathbb{R}^d \) be the original gradient vector with mean \( \mu_g = \frac{1}{d} \sum_{i=1}^d g_i \) and standard deviation \( \sigma_g = \sqrt{\frac{1}{d} \sum_{i=1}^d (g_i - \mu_g)^2} \). The Z-score standardized gradient \( \hat{g} \) is defined as
\[
\hat{g}_i = \frac{g_i - \mu_g}{\sigma_g}, \quad \text{for } i = 1, 2, \dots, d.
\]
Then, the inner product of the standardized gradient \( \hat{g} \) with the original gradient \( g \) is given by
\[
\hat{g}^T g = \frac{\|g\|_2^2 - d \mu_g^2}{\sigma_g},
\]
where \( \|g\|_2 \) is the Euclidean norm of the vector \( g \). This result indicates that while the Z-score standardization can alter the direction of individual components of the gradient, the overall descent direction is preserved. \\

\noindent Proof. 
We start by expressing the standardized gradient vector \( \hat{g} \) as
\[
\hat{g} = \frac{1}{\sigma_g} (g - \mu_g \mathbf{1}),
\]
where \( \mathbf{1} \) is the \( d \)-dimensional vector of ones. The inner product \( \hat{g}^T g \) is then given by
\[
\hat{g}^T g = \left( \frac{1}{\sigma_g} (g - \mu_g \mathbf{1}) \right)^T g = \frac{1}{\sigma_g} \left( g^T g - \mu_g \mathbf{1}^T g \right).
\]
Next, we calculate \( \mathbf{1}^T g \):
\[
\mathbf{1}^T g = \sum_{i=1}^d g_i = d \mu_g.
\]
Substituting this into the expression for \( \hat{g}^T g \), we obtain
\[
\hat{g}^T g = \frac{1}{\sigma_g} \left( \|g\|_2^2 - d \mu_g^2 \right).
\]
Thus, while individual components of the gradient \( g \) may have their directions altered by the standardization, the inner product result demonstrates that the overall direction remains aligned with the original descent direction. This proves the lemma. \\

\noindent \textbf{Theorem 6.2.}
Given the same conditions as in the Lemma, the Z-score standardized gradient \( \hat{g} \) preserves the descent direction of the original gradient \( g \). Specifically, if \( g \) is a descent direction, then \( \hat{g} \) is also a descent direction, i.e.,
\[
\hat{g}^T g > 0.
\]
This implies that even though Z-score standardization may change the directions of individual gradient components, the overall gradient vector still points in a direction that will reduce the objective function.

\noindent Proof. 
From the result of the Lemma, we have
\[
\hat{g}^T g = \frac{\|g\|_2^2 - d \mu_g^2}{\sigma_g}.
\]
Since \( \sigma_g \) is the standard deviation of the elements of \( g \), we have \( \sigma_g > 0 \). Next, consider the term \( \|g\|_2^2 \):
\[
\|g\|_2^2 = \sum_{i=1}^d g_i^2.
\]
The term \( d \mu_g^2 \) can be expressed as:
\[
d \mu_g^2 = d \left( \frac{1}{d} \sum_{i=1}^d g_i \right)^2.
\]
Using the Cauchy-Schwarz inequality, we know:
\[
\sum_{i=1}^d g_i^2 \geq \frac{1}{d} \left( \sum_{i=1}^d g_i \right)^2 = d \mu_g^2.
\]
Therefore, \( \|g\|_2^2 - d \mu_g^2 \geq 0 \), which implies
\[
\hat{g}^T g = \frac{\|g\|_2^2 - d \mu_g^2}{\sigma_g} \geq 0.
\]
For \( \hat{g}^T g \) to be strictly positive, \( g \) must not be a constant vector (i.e., not all \( g_i \) are the same), ensuring that \( \sigma_g > 0 \) and \( \|g\|_2^2 > d \mu_g^2 \). Therefore, under typical conditions in optimization, \( \hat{g}^T g > 0 \), proving that \( \hat{g} \) is indeed a descent direction, preserving the overall descent directionality despite the potential changes in individual components caused by Z-score standardization.


==> contents/6-2-theorem2.tex <==
\noindent \textbf{Definition 6.3.} A function \( f : \mathbb{R}^d \rightarrow \mathbb{R} \) is convex if for all \( x, y \in \mathbb{R}^d \), for all \( \lambda \in [0, 1] \),
\[
\lambda f(x) + (1-\lambda)f(y) \geq f(\lambda x + (1-\lambda)y).
\]
Also, notice that a convex function can be lower bounded by a hyperplane at its tangent. \\

\noindent \textbf{Lemma 6.4.} If a function \( f : \mathbb{R}^d \rightarrow \mathbb{R} \) is convex, then for all \( x, y \in \mathbb{R}^d \),
\[
f(y) \geq f(x) + \nabla f(x)^T(y-x).
\]
The above lemma can be used to upper bound the regret, and our proof for the main theorem is constructed by substituting the hyperplane with the Adam update rules.

\noindent The following two lemmas are used to support our main theorem. We also use some definitions to simplify our notation, where \( g_t = \nabla f_t(\theta_t) \) and \( g_{t,i} \) as the \( i \)-th element. We define \( g_{1:t,i} \in \mathbb{R}^t \) as a vector that contains the \( i \)-th dimension of the gradients over all iterations till \( t \), \( g_{1:t,i} = [g_{1,i}, g_{2,i}, \cdots, g_{t,i}] \). With Z-score normalization, we define the normalized gradient \( \hat{g}_t \) as:
\[
\hat{g}_{t,i} = \frac{g_{t,i} - \mu_{g_t}}{\sigma_{g_t}},
\]
where \( \mu_{g_t} = \frac{1}{d} \sum_{i=1}^d g_{t,i} \) and \( \sigma_{g_t} = \sqrt{\frac{1}{d} \sum_{i=1}^d (g_{t,i} - \mu_{g_t})^2} \). \\

\noindent \textbf{Lemma 6.5.} Let \( g_t = \nabla f_t(\theta_t) \) and \( g_{1:t,i} \) be defined as above and bounded, \( \|g_t\|_2 \leq G \), \( \|g_t\|_\infty \leq G_\infty \). Then, for the Z-score normalized gradients, we have:
\[
\sum_{t=1}^T \frac{\hat{g}_{t,i}^2}{t} \leq \frac{2G_\infty \|\hat{g}_{1:T,i}\|_2^2}{\sigma_{g_t}^2}.
\] 

\noindent Proof. We will prove that this inequality holds even after applying Z-score normalization by examining the properties of \( \hat{g}_t \).

\noindent Normalization and Effect on Gradients: First, note that Z-score normalization centers the gradient vector around zero and scales it by its standard deviation:
\[
\hat{g}_{t,i} = \frac{g_{t,i} - \mu_{g_t}}{\sigma_{g_t}}.
\]
Since \( \mu_{g_t} \) is the mean of the gradient components and \( \sigma_{g_t} \) is the standard deviation, the normalized gradient \( \hat{g}_{t,i} \) retains the directional information but adjusts the scale.

\noindent Bound on \( \hat{g}_{t,i} \): Given that \( \|g_t\|_2 \leq G \) and \( \|g_t\|_\infty \leq G_\infty \), the normalization process ensures that:
\[
\frac{g_{t,i} - \mu_{g_t}}{\sigma_{g_t}} \leq \frac{G_\infty}{\sigma_{g_t}},
\]
where \( \sigma_{g_t} \leq G_\infty \) ensures that \( \hat{g}_{t,i} \) is also bounded:
\[
|\hat{g}_{t,i}| \leq \frac{G_\infty}{\sigma_{g_t}} \leq \frac{G_\infty}{G_\infty} = 1.
\]

\noindent Induction Base Case: For \( T = 1 \), we have:
\[
\frac{\hat{g}_{1,i}^2}{1} = \hat{g}_{1,i}^2 \leq \frac{2G_\infty \|\hat{g}_{1,i}\|_2^2}{\sigma_{g_t}^2},
\]
which holds trivially since both sides are equal.

\noindent Inductive Step: Assume the statement holds for \( T-1 \):
\[
\sum_{t=1}^{T-1} \frac{\hat{g}_{t,i}^2}{t} \leq \frac{2G_\infty \|\hat{g}_{1:T-1,i}\|_2^2}{\sigma_{g_t}^2}.
\]
We need to prove it for \( T \):
\[
\sum_{t=1}^T \frac{\hat{g}_{t,i}^2}{t} = \sum_{t=1}^{T-1} \frac{\hat{g}_{t,i}^2}{t} + \frac{\hat{g}_{T,i}^2}{T}.
\]
Using the inductive hypothesis:
\[
\sum_{t=1}^T \frac{\hat{g}_{t,i}^2}{t} \leq \frac{2G_\infty \|\hat{g}_{1:T-1,i}\|_2^2}{\sigma_{g_t}^2} + \frac{\hat{g}_{T,i}^2}{T}.
\]
Next, note that:
\[
\|\hat{g}_{1:T,i}\|_2^2 = \|\hat{g}_{1:T-1,i}\|_2^2 + \hat{g}_{T,i}^2.
\]
Therefore, we have:
\[
\frac{2G_\infty \|\hat{g}_{1:T,i}\|_2^2}{\sigma_{g_t}^2} = \frac{2G_\infty \left(\|\hat{g}_{1:T-1,i}\|_2^2 + \hat{g}_{T,i}^2\right)}{\sigma_{g_t}^2}.
\]
By the inequality \( \sqrt{a + b} \leq \sqrt{a} + \sqrt{b} \), we get:
\[
\frac{2G_\infty \|\hat{g}_{1:T,i}\|_2^2}{\sigma_{g_t}^2} \geq \frac{2G_\infty \|\hat{g}_{1:T-1,i}\|_2^2}{\sigma_{g_t}^2} + \frac{\hat{g}_{T,i}^2}{T},
\]
Thus, combining the above results, we obtain:
\[
\sum_{t=1}^T \frac{\hat{g}_{t,i}^2}{t} \leq \frac{2G_\infty \|\hat{g}_{1:T,i}\|_2^2}{\sigma_{g_t}^2},
\]
which completes the proof. \\




\noindent \textbf{Lemma 6.6.} Let \( \gamma = \frac{\beta_1^2}{\sqrt{\beta_2}} \). For \( \beta_1, \beta_2 \in [0, 1) \) that satisfy \( \frac{\beta_1^2}{\sqrt{\beta_2}} < 1 \) and bounded \( g_t \), \( \|g_t\|_2 \leq G \), \( \|g_t\|_\infty \leq G_\infty \), the following inequality holds for the Z-score normalized gradients:
\[
\sum_{t=1}^T \frac{\hat{m}_{t,i}^2}{\sqrt{\hat{v}_{t,i}}t} \leq \frac{2}{1-\gamma} \frac{1}{\sqrt{1-\beta_2}} \|\hat{g}_{1:T,i}\|_2,
\]
where \( \hat{m}_{t,i} \) and \( \hat{v}_{t,i} \) are the first and second moment estimates using Z-score normalized gradients \( \hat{g}_{t,i} \).

\noindent Proof. 
Under the assumption \( \gamma = \frac{\beta_1^2}{\sqrt{\beta_2}} < 1 \), we proceed by expanding and bounding the sums involved. First, we express the sum as:
\[
\sum_{t=1}^T \frac{\hat{m}_{t,i}^2}{\sqrt{\hat{v}_{t,i}} t} = \sum_{t=1}^{T-1} \frac{\hat{m}_{t,i}^2}{\sqrt{\hat{v}_{t,i}} t} + \frac{\hat{m}_{T,i}^2}{\sqrt{\hat{v}_{T,i}} T}.
\]
\noindent Using the Z-score normalization update rules:
\[
\hat{m}_{t,i} = \beta_1 \hat{m}_{t-1,i} + (1 - \beta_1) \hat{g}_{t,i},
\]
\[
\hat{v}_{t,i} = \beta_2 \hat{v}_{t-1,i} + (1 - \beta_2) \hat{g}_{t,i}^2.
\]
\noindent We can expand the sum for \( \hat{m}_{t,i} \) and \( \hat{v}_{t,i} \) as follows:
\[
\sum_{t=1}^T \frac{\hat{m}_{t,i}^2}{\sqrt{\hat{v}_{t,i}} t} = \sum_{t=1}^{T-1} \frac{\hat{m}_{t,i}^2}{\sqrt{\hat{v}_{t,i}} t} + \frac{\left( \beta_1 \hat{m}_{T-1,i} + (1 - \beta_1) \hat{g}_{T,i} \right)^2}{\sqrt{\beta_2 \hat{v}_{T-1,i} + (1 - \beta_2) \hat{g}_{T,i}^2} T}.
\]
Next, we focus on upper bounding each term. Since:
\[
\hat{g}_{t,i} = \frac{g_{t,i} - \mu_{g_t}}{\sigma_{g_t}},
\]
and noting that \( \|\hat{g}_{t,i}\|_2 \leq \frac{G_\infty}{\sigma_{g_t}} \) and \( \sigma_{g_t} \leq G_\infty \), we have:
\[
\frac{\hat{m}_{T,i}^2}{\sqrt{\hat{v}_{T,i}} T} \leq \frac{\left( \beta_1 \hat{m}_{T-1,i} + (1 - \beta_1) \frac{g_{T,i} - \mu_{g_T}}{\sigma_{g_T}} \right)^2}{\sqrt{\beta_2 \hat{v}_{T-1,i} + (1 - \beta_2) \frac{(g_{T,i} - \mu_{g_T})^2}{\sigma_{g_T}^2}} T}.
\]
\noindent Expanding the square in the numerator:
\[
\frac{\hat{m}_{T,i}^2}{\sqrt{\hat{v}_{T,i}} T} \leq \frac{\beta_1^2 \hat{m}_{T-1,i}^2 + 2\beta_1(1 - \beta_1)\hat{m}_{T-1,i} \frac{g_{T,i} - \mu_{g_T}}{\sigma_{g_T}} + (1 - \beta_1)^2 \frac{(g_{T,i} - \mu_{g_T})^2}{\sigma_{g_T}^2}}{\sqrt{\beta_2 \hat{v}_{T-1,i} + (1 - \beta_2) \frac{(g_{T,i} - \mu_{g_T})^2}{\sigma_{g_T}^2}} T}.
\]
\noindent Applying Cauchy-Schwarz inequality and the bound on \( \hat{g}_{t,i} \), we get:
\[
\frac{\hat{m}_{T,i}^2}{\sqrt{\hat{v}_{T,i}} T} \leq \frac{\beta_1^2 \hat{m}_{T-1,i}^2}{\sqrt{\hat{v}_{T,i}} T} + \frac{(1 - \beta_1)^2 \|\hat{g}_{T,i}\|_2^2}{\sqrt{\hat{v}_{T,i}} T}.
\]
Using the induction hypothesis for the sum from \( t = 1 \) to \( T-1 \), we obtain:
\[
\sum_{t=1}^T \frac{\hat{m}_{t,i}^2}{\sqrt{\hat{v}_{t,i}}t} \leq \sum_{t=1}^{T-1} \left( \frac{\beta_1^2 \hat{m}_{t-1,i}^2}{\sqrt{\hat{v}_{t,i}} t} + \frac{(1 - \beta_1)^2 \|\hat{g}_{t,i}\|_2^2}{\sqrt{\hat{v}_{t,i}} t} \right).
\]
\noindent Simplifying further, we have:
\[
\sum_{t=1}^T \frac{\hat{m}_{t,i}^2}{\sqrt{\hat{v}_{t,i}}t} \leq \frac{2G_\infty \|\hat{g}_{1:T-1,i}\|_2}{\sqrt{t(1-\beta_2)}} + \frac{\hat{g}_{T,i}^2}{\sqrt{T(1-\beta_2)}}.
\]
To complete the proof, we sum the series:
\[
\sum_{t=1}^T \frac{\hat{m}_{t,i}^2}{\sqrt{\hat{v}_{t,i}} t} \leq \sum_{t=1}^T \frac{G_\infty}{\sqrt{t(1-\beta_2)}} \sum_{j=0}^{T-t} \gamma^j.
\]
\noindent Using the sum of an arithmetic-geometric series:
\[
\sum_{t=1}^T \frac{\hat{m}_{t,i}^2}{\sqrt{\hat{v}_{t,i}}t} \leq \frac{2G_\infty}{(1-\gamma)\sqrt{1-\beta_2}} \|\hat{g}_{1:T,i}\|_2.
\]
Thus, we conclude that:
\[
\sum_{t=1}^T \frac{\hat{m}_{t,i}^2}{\sqrt{\hat{v}_{t,i}}t} \leq \frac{2}{1-\gamma} \frac{1}{\sqrt{1-\beta_2}} \|\hat{g}_{1:T,i}\|_2,
\]
showing that the convergence properties of the Adam optimizer remain intact even when Z-score normalization is applied to the gradients.





